The Last-Iterate Convergence Rate of Optimistic Mirror Descent in Stochastic Variational Inequalities

In this paper, we analyze the local convergence rate of optimistic mirror descent methods in stochastic variational inequalities, a class of optimization problems with important applications to learning theory and machine learning. Our analysis reveals an intricate relation between the algorithm's rate of convergence and the local geometry induced by the method's underlying Bregman function. We quantify this relation by means of the Legendre exponent, a notion that we introduce to measure the growth rate of the Bregman divergence relative to the ambient norm near a solution. We show that this exponent determines both the optimal step-size policy of the algorithm and the optimal rates attained, explaining in this way the differences observed for some popular Bregman functions (Euclidean projection, negative entropy, fractional power, etc.).

==> BregReg.tex <==
%----------------------------------------------------------------------
%%% REGULARITY
%----------------------------------------------------------------------
% !TEX root = ./Main.tex


The Bregman divergence involved in the algorithm plays a crucial part in the convergence rate, both in practice and in theory as we develop next. In order to capture the observed behaviors, we introduce the notion of Legendre exponent which will play a central role in our analysis.

\subsection{Practical motivation}

Let us consider a simple $1D$ example with $\points=[0,+\infty)$ and  $\vecfield(\point) = \point$; the solution of the associated variational inequality is thus $\sol=0$. It is direct to see that $\vecfield$ is $\lips=1$ Lipschitz continuous and $\strong=1$ strongly monotone. 

Let us consider three Bregman regularizers on $\points$:
\begin{itemize}
    \item (Euclidean)  $\hreg^{(euc)}(\point) = \point^{2}/2$, which satisfies $\breg(\sol,\point) = \point^{2}/2$,
and
$\proxof{\point}{\dpoint} = [\point + \dpoint]_+$ for any $\point\in[0,+\infty), \dpoint\in\R$;
    \item (Entropy)  $\hreg^{(ent)}(\point) = \point \log\point$,  which satisfies $\breg(\sol,\point) = \point$,
and
$\proxof{\point}{\dpoint} = \point \exp(\dpoint)$ for all $\point\in(0,\infty)$, $\dpoint\in\R$;
    \item (Square root)  $\hreg^{(sqr)}(\point) = \point-2\sqrt{\point}$, which satisfies $\breg(\sol,\point) = \sqrt{\point}$,
and
$\proxof{\point}{\dpoint} = 1/(1/\sqrt{\point} - \dpoint)^2$ for any $\point\in(0,\infty)$, $\dpoint\in\R$.
\end{itemize}


For each of these Bregman regularizers, we run \ac{OMD} initialized with $\init=\initlead=0.1$, $\noise$ an i.i.d. Gaussian noise process with mean $0$ and variance $\sdev^2=1e-4$. We choose our stepsize sequence as 
\begin{align}
    \curr[\step] = \frac{1}{\run^\eta}
\end{align}
with $\eta=0.7$. 


\begin{figure}
    \centering
 \begin{subfigure}[t]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figs/logx_ite.pdf}
         \caption{Iterates behavior}
         \label{fig:comp-ite}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figs/Dx_ite.pdf}
         \caption{Bregman divergence to the solution}
         \label{fig:comp-breg}
     \end{subfigure}
    \caption{Comparison of Bregman regularizers' behaviors in terms of iterates and divergence (averaged over 100 runs) }
    \label{fig:comp}
\end{figure}

In \cref{fig:comp}, we report for these three Bregman regularizers the decrease of $\curr[\state]$ to $\sol=0$ by plotting (a) $\curr[\state]$ and (b) $\breg(\sol,\curr[\state])$ averaged over $100$ runs. We observe that no matter the quantity investigated the convergence rates are different. 

In particular, we observed by running this experiments for various values of $\eta$ a general trend as follows:\\
\begin{tabular}{r|c|c|c}
Bregman  Regularizer   $\hreg$  & Euclidean & Entropy & Square root \\
Bregman  Divergence  to the solution $\breg(\sol,\point)$   &  $0.5\point^2$  &  $\point$ & $\sqrt{\point}$\\
Observed rate\footnotemark of $\breg(\sol,\curr[\state])$    &  $\bigoh{\frac{1}{\run^\eta}}$  &  $\bigoh{\frac{1}{\run^{1-\eta}}}$  & $\bigoh{\frac{1}{\run^{(1-\eta)/3}}}$ 
\end{tabular}
\footnotetext{The actual rates computed by linear regression on right part of \cref{fig:comp} (b) were: $1/\run^{0.756}$ (for $1/\run^{0.7}$) in the Euclidean case, $1/\run^{0.293}$ (for $1/\run^{0.3}$) in the Entropy case, and $1/\run^{0.097}$ (for $1/\run^{0.1}$) in the Square root case.}

The rate in the Euclidean case seem to have another behavior as the two others which is not surprising. As for the two others, we notice that $\breg(\sol,\point)/\point^2 = 1/\point = 1/\breg(\sol,\point)$ for the Entropy case while  $\breg(\sol,\point)/\point^2 = 1/\point^{3/2} = 1/ \breg(\sol,\point)^3$ for the square root case.  Thus, the rates seem to be controlled by the behavior of $\breg(\sol,\point)$ with respect to the Euclidean case.


%%% commented out from Franck's presentation :

% \subsection{Theoretical motivation}

% In terms of theory, a limitation of the use of strong monotonicity in non-Euclidean geometries is that we typically face descent inequalities of the form
% \begin{align}
% \tag{``informal'' descent}
%     \breg(\sol, \next)  \underset{\approx}{\leq} \breg(\sol, \curr) - \mu\curr[\step] \|\curr-\sol\|^2 + \dots .
% \end{align}

% The valuable information brought by the negative terms cannot be exploited in general due the the lack of lower bound of the euclidean error $\|\curr-\sol\|^2$ by the Bregman error $\breg(\sol, \curr)$. 


% \subsection{Legendre exponent}

% Motivated by the previous sections, we introduce a way to lower bound the euclidean error $\|\curr-\sol\|^2$ by a power of the Bregman error $\breg(\sol, \curr)$.

% \begin{definition}
% \label{def:Legendre}
% A Bregman regularizer $\hreg$ has \emph{Legendre exponent} $\leg\geq 0$ at $\sol$ if there is a convex neighborhood $\nhd$ of $\sol$ in $\points$  such that the associated Bregman divergence satisfies
%             \begin{equation*}
%                 \breg(\sol,\point)^{1 + \leg} \leq \frac{M}{2} \norm{ \point - \sol}^2 \quad \forall \point \in \nhd
%             \end{equation*}
%         for some $1\leq M<\infty$.
% \end{definition}


% \begin{remark}\label{rmk: alpha implies bound u}
%     A positive Legendre exponent $\leg > 0$ implies a bound on the size of $\nhd$. Using the strong convexity of $\hreg$ (\cref{lemma: strg cvx h}), for any $\point \in \nhd$,
%     \begin{equation*}
%       \breg(\sol,\point)^\leg \leq M\,.
%     \end{equation*}
%     % As a consequence, for any $\alpha \geq 0$,
%     % \begin{equation*}
%     %     0 \leq D(x^*, x) - \frac{1}{M}D(x^*, x)^{1+\alpha}\,.
%     % \end{equation*}
% \end{remark}



